Long-History User Transformers for Real-Time Ad Ranking

Long interaction histories are among the most informative inputs for click-through rate (CTR) prediction, yet in online advertising they collide with a hard serving constraint: ads must be scored within a few hundred milliseconds to enter the auction, which rules out running a large sequence encoder at request time. We describe how a production advertising system resolves this conflict by decoupling history encoding from real-time inference. A high-capacity offline transformer asynchronously encodes the user's full cross-surface interaction history into a compact representation cached in a feature store, while a lightweight runtime model combines this cached representation with the user's most recent events and the request context at serving time. The offline encoder is pre-trained autoregressively on large-scale interaction logs with a dual objective - feedback prediction and next-item prediction - and the two-stage architecture is then fine-tuned for CTR prediction on the target advertising surface. Offline, the split design recovers 72-80% of the quality of a full-history runtime transformer that would be too expensive to deploy, and the cached representation is robust enough to staleness to permit inexpensive refresh policies. In production A/B experiments, the system improves the primary ranking metric by +2.77% in search advertising and +2.1% on the Yandex Advertising Network, with revenue gains of +2.26% and +0.43% respectively - without increasing serving latency.

==> title_page/title.tex <==


\begin{titlepage}

\begin{center}
\vfill
%\framepage

\includegraphics[width=16cm,]{title_page/graph/01_Main_Logo_in_line_ENG_PANTONE.png}\\[1cm]
FACULTY OF COMPUTER SCIENCE\\
\ \\


\vfill
{
\huge Transformer model based on the user's story for advertising\\[3cm]


 

}

\begin{minipage}{0.4\textwidth}
		\begin{flushleft}
			\large
			\text{Author:}\\
			\large Vycheslav Ovchinnikov % Your name
		\end{flushleft}
	\end{minipage}
	~
	\begin{minipage}{0.4\textwidth}
		\begin{flushright}
			\large
			\text{Supervisor:}\\
			\large Maxim Kuzin% Your name
		\end{flushright}
	\end{minipage}

\vfill


Moscow\\
March 2026
\end{center}

\end{titlepage}

\newpage
